Practical algorithms and experimentally validated incentives for equilibrium-based fair division (A-CEEI)

Approximate Competitive Equilibrium from Equal Incomes (A-CEEI) is an equilibrium-based solution concept for fair division of discrete items to agents with combinatorial demands. In theory, it is known that in asymptotically large markets: 1. For incentives, the A-CEEI mechanism is Envy-Free-but-for-Tie-Breaking (EF-TB), which implies that it is Strategyproof-in-the-Large (SP-L). 2. From a computational perspective, computing the equilibrium solution is unfortunately a computationally intractable problem (in the worst-case, assuming $\textsf{PPAD}\ne \textsf{FP}$). We develop a new heuristic algorithm that outperforms the previous state-of-the-art by multiple orders of magnitude. This new, faster algorithm lets us perform experiments on real-world inputs for the first time. We discover that with real-world preferences, even in a realistic implementation that satisfies the EF-TB and SP-L properties, agents may have surprisingly simple and plausible deviations from truthful reporting of preferences. To this end, we propose a novel strengthening of EF-TB, which dramatically reduces the potential for strategic deviations from truthful reporting in our experiments. A (variant of) our algorithm is now in production: on real course allocation problems it is much faster, has zero clearing error, and has stronger incentive properties than the prior state-of-the-art implementation.

==> obsolete.tex <==
\label{subsec:perform-of-ours}
\begin{table}[t]
    \centering

    \begin{tabular}{|c|cc|cc|cc|}
        \hline
        \multirow{2}{*}{Instance} & \multicolumn{2}{c|}{Size}                     & \multicolumn{2}{c|}{Solution} & \multicolumn{2}{c|}{Statistics}                                                  \\ \cline{2-7} 
        & \multicolumn{1}{c|}{$n$} & $m$ & \multicolumn{1}{c|}{$\alpha$} & $\beta$ & \multicolumn{1}{c|}{Avg. \# iterations} & Avg. time \\ \hline

        \multirow{3}{*}{Toronto Law in Fall 2019} & \multicolumn{1}{c|}{\multirow{3}{*}{435}} & \multirow{3}{*}{171} & \multicolumn{1}{c|}{0} & 0.02 &  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} $206+171.5$ (regular)\\ $206+186.8$ (strong)\end{tabular}}  &  \begin{tabular}[c]{@{}l@{}}1min 31s (regular)\\ 1min 45s (strong)\end{tabular}    \\ \cline{4-7}

        & \multicolumn{1}{c|}{} & & \multicolumn{1}{c|}{0} & 0.04 &  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} $206+23.4$ (regular)\\ $206+19.7$ (strong)\end{tabular}}  & \begin{tabular}[c]{@{}l@{}} 42s (regular)\\ 44s (strong)\end{tabular}    \\ \hline

        \multirow{3}{*}{Toronto Law in Fall 2021} & \multicolumn{1}{c|}{\multirow{3}{*}{468}} & \multirow{3}{*}{156} & \multicolumn{1}{c|}{0} & 0.02 &  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} $202+95.5$ (regular)\\ $202+99.5$ (strong)\end{tabular}}  &  \begin{tabular}[c]{@{}l@{}} 3min 48s (regular)\\ 4min \;\,5s (strong)\end{tabular}  \\ \cline{4-7}
        
            & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{0} & 0.04 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} $202+43.1$ (regular)\\ $202+44.5$ (strong)\end{tabular}} & \begin{tabular}[c]{@{}l@{}} 2min 44s (regular)\\ 2min 51s (strong)\end{tabular} \\ \hline

        \multirow{3}{*}{Toronto Law in Fall 2022} & \multicolumn{1}{c|}{\multirow{3}{*}{473}} & \multirow{3}{*}{181} & \multicolumn{1}{c|}{0} & 0.02 &  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} $202+192.6$ (regular)\\ $202+206.6$ (strong)\end{tabular}}  &  \begin{tabular}[c]{@{}l@{}} 4min 53s (regular)\\ 5min 16s (strong)\end{tabular} \\ \cline{4-7}
        
            & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{0} & 0.04 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} $202+47.2$ (regular)\\ $202+53.7$ (strong)\end{tabular}}  &  \begin{tabular}[c]{@{}l@{}} 2min 23s (regular)\\ 2min 30s (strong)\end{tabular} \\ \hline

        \multirow{3}{*}{OR data\footnote{budgets are all less than $1$}} & \multicolumn{1}{c|}{\multirow{3}{*}{1700}}            &   \multirow{3}{*}{344}        & \multicolumn{1}{c|}{0} & 0.02 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} $131+86.4$ (regular)\\ $131+91.1$ (strong)\end{tabular}}              &   \begin{tabular}[c]{@{}l@{}} 7min 30s (regular)\\ 9min 19s (strong)\end{tabular}   \\ \cline{4-7}
        & \multicolumn{1}{c|}{}            &            & \multicolumn{1}{c|}{0} & 0.04 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} $131+49.2$ (regular)\\ $131+43.8$ (strong)\end{tabular}}              &   \begin{tabular}[c]{@{}l@{}} 6min \;\,4s (regular)\\ 7min 19s (strong)\end{tabular}  \\ \hline

        \multirow{3}{*}{large.in (Columbia?)} & \multicolumn{1}{c|}{\multirow{3}{*}{1119}}            &   \multirow{3}{*}{317}         & \multicolumn{1}{c|}{0} & 0.02 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} $252+120.6$ (regular)\\ $252+219.8$ (strong)\end{tabular}}              &   \begin{tabular}[c]{@{}l@{}} 4min 40s (regular)\\ 7min 2s (strong)\end{tabular}    \\\cline{4-7}
        
        & \multicolumn{1}{c|}{}            &          & \multicolumn{1}{c|}{0} & 0.04 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} $252+27.0$ (regular)\\ $252+75.3$ (strong)\end{tabular}}              &     \begin{tabular}[c]{@{}l@{}} 2min 25s (regular)\\ 4min \;\,3s (strong)\end{tabular}  \\\hline
        
        \multirow{3}{*}{giant.in (Columbia)} & \multicolumn{1}{c|}{\multirow{3}{*}{2385}}            &   \multirow{3}{*}{658}         & \multicolumn{1}{c|}{0} & 0.02 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} $642+286.2$ (regular)\\ $642+492.7$ (strong)\end{tabular}}              &   \begin{tabular}[c]{@{}l@{}} 30min \;\,8s (regular)\\ 45min 18s (strong)\end{tabular}    \\\cline{4-7}
        &    \multicolumn{1}{c|}{}         &          & \multicolumn{1}{c|}{0} & 0.04 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}l@{}} $642+90.7$ (regular)\\ $642+180.6$ (strong)\end{tabular}}              &   \begin{tabular}[c]{@{}l@{}} 18min 42s (regular)\\ 26min 43s (strong)\end{tabular}    \\\hline
    \end{tabular}
    % compressed\_big.in & 435 & 171 & & & 
    \caption{Computational results of our algorithm. We guarantee (strong) EF-TB for the solutions. For each instance, we count the average number of iterations for the warm start and our algorithm separately, where the left of the $+$ signs represent the numbers for warm starts.}
    \label{tbl:compute-results}
\end{table}

In several instances from several schools, our algorithm can find an A-CEEI solution satisfying (strong) EF-TB that has zero clearing error and mild budget perturbation. We show the statistics for the instances, the solutions, and the running time in Table~\ref{tbl:compute-results}. 





\subsubsection{Algorithms in Consideration}

\paragraph{Discrete Tatonnement.} As previously remarked, discrete tatonnement is our basic algorithm by setting parameter $\epsilon$ to $0$. 



\paragraph{Discrete Tatonnement with budget perturbation checks.} In this algorithm, we do two modifications on Algorithm~\ref{alg:tatonnement}:
\begin{enumerate}
    \item we only execute steps 2 and 3 with some probability $p$; and 
    \item we update the price by adding the excess demand without budget perturbation, i.e. by $\vc{p}\gets \vc{p} + \delta \vc{\tilde{z}}(\vc{u}, \vc{c}, \vc{p}, \vc{b_0})$.
\end{enumerate}







\subsubsection{Comparing with the baseline}
\Aviad{I think that throughout the paper we should call it ``optimized/optimal/smart budget perturbations'' to distinguish from the randomness of $b_0$, and also from the second (aka after finding a Kakutani fixed point of the correspondence)  random perturbations in the proof of existence.}
We compare our (basic) algorithm with the tabu search of the first stage of the baseline \Aviad{We should explain why we're only comparing to first stage} in this subsection. Compared to the first stage of the baseline, our basic algorithm makes the following two major modifications: 
\begin{itemize}
    % \item[(a)] removing individual price adjustments, 
    \item[(a)] using fixed step size and giving up exploring multiple neighbors\Aviad{With the warm start and binary search improvements, are we really using a fixed step size?} \Ruiquan{This part is changed to the difference between our basic algorithm and the baseline.}%and removing tabu search, and
    \item[(b)] adding budget perturbation. 
\end{itemize}
To present the significance of the modifications, we shall consider the following four algorithms:
\begin{itemize}
    \item[(i)] the first stage of the baseline,
    % \item[(ii)] the first stage of the baseline without individual price adjustments, which modifies (i) with (a),
    \item[(ii)] discrete tatonnement, which modifies (i) with (a), 
    \item[(iii)] our basic algorithm,
    \item[(iv)] our algorithm.
    % \item[(v)] tatonnement with budget perturbation checks.
\end{itemize}






On the other hand, we acknowledge that our algorithm cannot guarantee to monotonically reduce the clearing error. This is contrary to the design of tabu search of~\cite{OthmanSB10,BudishCKO17} of which each step picks the price with optimal clearing error within a large neighborhood. However, it should not be a serious issue to tatonnement-based algorithms, because of the following artificial example of a tatonnement run that has non-monotonic clearing errors but finally finds a zero-error solution. 
\begin{example}
    Consider the economy consisting of 
    \begin{itemize}
        \item 3 courses: $\{a,b,c\}$ with capacities $(1,0,0)$;
        \item 1 student with single-minded demand ${a,b,c}$;
    \end{itemize}
    Further, consider we run discrete tatonnement starting at prices $(0.4,0.3,0.3)$ with fixed step size $\delta = 0.01$. 
    
    In the beginning, the student can afford the bundle and the excess demand is thus $(0,1,1)$. Then, the algorithm alternates as follows:
    \begin{itemize}
        \item increasing $p_b,p_c$ by $\delta$, after which the sum of the prices becomes $1+2\delta$ and the excess demand becomes $(-1, 0, 0)$;
        \item two steps of decreasing $p_a$ by $\delta$, after which the sum of the prices becomes $1$ and the excess demand becomes $(0, 1, 1)$.
    \end{itemize}
    After 20 such alternations, the prices become $(0, 0.5, 0.5)$ and the excess demand becomes $(0,1,1)$. The algorithm proceeds another step to prices $(0, 0.51, 0.51)$. At this time, because the price of $a$ is $0$, the under-demand of $a$ should be clipped and the algorithm finds a zero-clearing error solution.  
\end{example}









We have a few explanations for this phenomenon:
\begin{enumerate}
    \item First~\cite{OthmanSB10} compared Algorithms Benchmark and Vanilla in terms of number of iterations. For larger instances (\cite{OthmanSB10} only considered smaller \Ruiquan{random} instances of size \Aviad{TBD} \Ruiquan{with 50 courses and 250 students}), the total {\em running time} of individual price adjustments becomes quite long because each iteration is slower (see Table~\ref{tab:TBD})%
    \footnote{We note that in the experiments we actually measure a proprietary variant of the benchmark algorithm whose time-per-iteration has been heavily optimized. We also note that when we tried to combine individual  price adjustments with optimized budget perturbations, the computational overhead of individual price adjustments was even worse.}. 
    
    \item However, time-per-iteration tells only half of the story.
    As we show in Figure~\ref{fig:progress-of-algos-error}, even when counting only the number of iterations\Ruiquan{Should it be the running time?}, Vanilla initially outperforms Benchmark! Eventually the more elaborate Benchmark does win when measuring against number of iterations\Ruiquan{Same above?}, but this advantage only kicks in long after our algorithms (Basic and Fast).
    Since we aim for (and achieve) faster algorithms, we're more interested in this initial phase where Vanilla outperforms Benchmark for number of iterations.
    
    \item Finally, why does Vanilla (initially) outperform Benchmark even in terms of number of iterations? We postulate that this is because Vanilla can efficiently force the search out of local minima (of clearing error). Indeed the clearing error does not monotonically decrease throughout the run of our algorithm!\Ruiquan{It seems now we do not have such results (in terms of the number of iterations). Long ago, when we run the tabu search with only gradient steps, we can observe it but it was not very significant. }
\end{enumerate}



\section{Understanding manipulations via case studies}
\Aviad{I think we should keep a copy of this section for our record, but significantly simplify this section to highlight only the 2 courses per example, and not worry too much about actual numbers, etc}


How can strategic students manipulate SP-L  mechanisms in realistic instances? 
To really understand the nature of manipulations found by the algorithm, in this section we use qualitative analysis to zoom in on specific manipulations; we will describe one case study for each variant of our algorithm (no EF-TB, regular EF-TB, and strong EF-TB). Of course, each case study may not be representative of all possible manipulations. However, we find this methodology quite helpful for gaining intuition. In particular, we were able to use the case study for EF-TB to extract the simple manipulation described in the introduction, and propose the strong EF-TB criterion in response. 

\paragraph{5-additive utilities}
Unfortunately, the original preferences in the true instances are incredibly complicated, mostly due to various constraints imposed by the schools (e.g.~avoiding courses with conflicting meeting times, meeting minimum unit requirements, etc). 
To keep the case study analyses tractable, we repeat the manipulation finding experiments, but on modified preferences that ignore all those constraints and simply assume that the students utility is {\em 5-additive}, i.e.~each student wants the schedule of 5 courses that maximizes the total weight; here we use the original course weights reported by the students, but ignore all conflicts and requirements. Formally, for every student $i\in [n]$, the new utility function can be described by tuple $(\vc{w}',valid',req')$ where $\vc{w}'=(w_j)_{j\in [m]}$, and for every bundle $\vc{x}\in 2^{[m]}$,
    \begin{align*}
        valid'(\vc{x})&=\begin{cases}1&\|\vc{x}\|_1\le 5\\0&\|\vc{x}\|_1>5\end{cases}\\
        req'(\vc{x})&=0
    \end{align*}

%\subsection{Case studies on 5-addtive instance}

%In this section we analyze in detail several concrete examples where some students can increase their chance of getting their favorite course under the setting of resampled mechanism's randomness.

%\Qianfan{TBD- why 5-additive?}
  

\subsubsection*{Experimental setup}

% \Aviad{Say something about the choice of instances, e.g.~what school, etc.}
% \Qianfan{TBD - something has been mentioned before, some reorganization needed.}
The instance is the data from Fall 2020 of Tuck School of Business, which contains 40 courses and 283 students. As mentioned before, the utilities in this instance lies in the range of $[10^{-3}, 400]$. Following is the plot of weight distribution in the instance.

\begin{figure}[H]
    \centering
    \includegraphics[scale=0.6]{img_instances/s3-tuck-fall-2020.inall_courses_analysis.pdf}
    \caption{Weight distribution of~\texttt{s3-tuck-fall-2020.in}}
\end{figure}

As you can see, there are clearly four classes of weights, which is actually a consequence of the bidding language they used. Students will label courses they want with four classes: favourite, great, good, fair \Aviad{Why are weights not completely determined by these 4 classes?}. And weight class are greatly separated.



As an example, following is the raw data of weight vector from student 76's utility classified to four classes, where each tuple $(c_i,w_i)$ indicates that student 76's weight for course $c_i$ is $w_i$.
\begin{verbatim}
[(8, 360.0), 
 (13, 3.15), (10, 2.55), (12, 1.95), (9, 1.35), 
 (29, 0.315), (28, 0.255), (22, 0.0975), (27, 0.0675),
 (23, 0.01332), (1, 0.01152), (2, 0.00984), (37, 0.00408), (36, 0.00324), (0, 0.00234)]
\end{verbatim}

\subsection{No EF-TB constraints case study}%: student 76's manipulation}

\Qianfan{TBD- new reasoning here}

We first investigate profitable manipulations in the 5-additive instance without EF-TB constraints at all.
Results show that without EF-TB constraints, very simple profitable manipulation exists, which even remains profitable to many students under the setting of resampled population.
%Nevertheless, we start our experiment from analyze a manipulation for student 76 in the the resampled randomness setting.

\paragraph{The manipulation}

The environment is mostly the same to the one in the last section, except that when computing budget perturbations, we ignore all EF-TB constraints defined by initial budgets.
And we are now looking at a different student, student 76.


The manipulation we found is simple -- to report course 2 as the second favourite course, i.e.,  
\begin{verbatim}
[(8, 360.0), 
 (2, 10.00), (13, 3.15), (10, 2.55), (12, 1.95), (9, 1.35), 
 (29, 0.315), (28, 0.255), (22, 0.0975), (27, 0.0675),
 (23, 0.01332), (1, 0.01152), (37, 0.00408), (36, 0.00324), (0, 0.00234)]
\end{verbatim}

The distributions of the utility from reporting these two utility profiles are shown in the following figure, where $\mathcal{D}_{76}$ is the utility distribution from reporting truthfully, and $\mathcal{D}_{76}'$ is the utility distribution from reporting the manipulation.
    
  \begin{figure}[H]
    \centering
    \includegraphics[scale=0.6]{img_case_studies/SP_s3-tuck-fall-2020-5-additive.in_0_300_0.0005_0.01_5000_5_2_1_0_True_0.0_equalbudgets_uniquesol_noEFTB_student76.pickle.pdf}
  \end{figure}  
\Qianfan{
  $p=1.4\times 10^{-221}.$}

In the analysis, we still make same simplifications to the last section, i.e., fixing a realization for initial budgets and do a local analysis.
  \paragraph{Prices \& capacities:} 
    The following table contains the prices and capacities of relevant courses.
    \begin{table}[H]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
    \hline
      & {\bf 1}  & {\bf 2} & {\bf 8} & {\bf 29} & others    \\ \hline
    Market-clearing price $\vc{p^*}$ & 10 & 5 & 10195  & 425  & 0 \\ \hline
    Remaining capacity (locally) & 1 & 1 & 1 & 1 & $>1$ \\ \hline
    \end{tabular}
    \end{table}

  \paragraph{Preferences, budgets, and possible allocations (irrelevant courses omitted):}     In the table below we describe the budgets and preferences of the relevant students.

    \begin{table}[H]
    \centering
    \begin{tabular}{|c|c|c|l|}
    \hline
                & Preferences                                                         & Initial budget $\vc{b_0}$ & Possible (allocation, budget perturbation)\\ \hline
    Student 76  & ${\bf 8}\gg 13 > 10 > 12 > 9 \gg {\bf 29} > \ast$                                                      & 10175          & \begin{tabular}[c]{@{}l@{}}($[{\bf 29},13,10,12,9]$, $0$)\\ ($[{\bf 8},13,10,12,9]$, $+20$)\end{tabular} \\ \hline
    \begin{tabular}[c]{@{}c@{}}\textbf{Student 76'}\\ (manipulated)\end{tabular} & ${\bf 8}\gg {\bf 2} > 13 > 10 > 12 > 9  \gg {\bf 29} >  \ast$                                                           & 10175 & \begin{tabular}[c]{@{}l@{}} ($[{\bf 2},13,10,12,9]$, $0$)\\ ($[{\bf 8},13,10,12,9]$, $+20$)\\ ($[{\bf 2},{\bf 8},13,10,12]$, $+25$)\end{tabular}         \\ \hline
    Student 134 & $23 \gg {\bf 8} > {\bf 29} > 34 > 19 \gg 33 > \ast$ & 10241  & \begin{tabular}[c]{@{}l@{}}($[23,{\bf 29},34,19,33]$, $-46$)\\ ($[23,{\bf 8},34,19,33]$, $0$)
    %\\ ($[23, {\bf 8},{\bf 29}, 34, 19]$, $+379$)
    \end{tabular}        \\ \hline
    Student 150  & \begin{tabular}[c]{@{}c@{}}${\bf 1} \gg 38 >  {\bf 8} > 28 > {\bf 2} > 3 > \ast$\end{tabular}                                                   & 10163  & \begin{tabular}[c]{@{}l@{}}($[{\bf 1},38,28,{\bf 2},3]$, $0$)\\ ($[{\bf 1},38,{\bf 8},28,3]$, $+42$)\\ ($[{\bf 1},38,{\bf 8},28,{\bf 2}]$, $+47$)\end{tabular}        \\ \hline
    \end{tabular}
    \end{table}
    
    
    

  \paragraph{Possible market-clearing allocations:}
  In the table below we present possible market-clearing allocations under different reported preferences.
  
    \begin{table}[H]
    \centering
    \begin{tabular}{|l|c|l|}
    \hline
    \multicolumn{1}{|c|}{Allocation}                                                                 & $\|b^*-b_0\|_1$ & \multicolumn{1}{|c|}{Comments}   \\ \hline
    \begin{tabular}[c]{@{}l@{}}76: $[{\bf 29},13,10,12,9]$    \\ 134: $[23,{\bf 8},34,19,33]$  \\  150: $[{\bf 1},38,28,{\bf 2},3]$\end{tabular} & $0+0+0=0$  &
    \begin{tabular}[c]{@{}l@{}}Chosen in the original case due to smaller l1 norm\\ No longer available in the manipulated case \end{tabular}  \\ \hline
    \begin{tabular}[c]{@{}l@{}}76: $[{\bf 8},13,10,12,9]$\\ 134: $[23,{\bf 29},34,19,33]$\\ 150 : $[{\bf 1},38,28,{\bf 2},3]$\end{tabular}           & $20+46+0=66$ &  Chosen in the manipulated case \\ \hline
    \begin{tabular}[c]{@{}l@{}}76: $[{\bf 2},13,10,12,9]$\\ 134: $[23,{\bf 29},34,19,33]$\\ 150 : $[{\bf 1},38,{\bf 8},28,3]$\end{tabular} & $0+46+42=88$ & \begin{tabular}[c]{@{}l@{}}Valid in the manipulated case while not chosen due to larger l1 norm\\ \end{tabular}  \\ \hline
    \end{tabular}
    \end{table}

    There are other students that also willing to give up course 2 just like student 150, but the cost on the l1 norm of budget change would be even higher. 
    Therefore, student 76 gets course 8 instead of 29 by reporting $2$ as the second favourite course.

% \paragraph{Some comments:}

% In the following experiments, we will further show that the simple manipulation (reporting $2$ as the second favourite course) is extremely powerful, in the sense that it remains profitable to many students even in the resampled population setting.


\subsection{Standard EF-TB constraints case study}%: student 134's manipulation}

\paragraph{The manipulation}
  %With  \texttt{5-additive} valuations, profitable manipulations still exist, but with much less frequency/significance compared to the manipulations with original valuations. The following is an illustrative case study for a profitable manipulation of student 71.
    %   \begin{figure}[h]
    %     \centering
    %     \includegraphics[scale=0.39]{SP_s3-tuck-fall-2020-additive-but-5.in_0_300_0.0005_0.01_100_20_2_1_0_True_0.0_equalbudgets_uniquesol_full.pickle.pdf}
    % \end{figure}

    Following is 134's weight tuples:
    \begin{verbatim}
        [(23, 360.0), 
         (8, 6.30), (29, 5.10), (34, 1.95), (19, 1.35), 
         (33, 0.1125), 
         (4, 0.0060), (7, 0.0045), (3, 0.0030)]
    \end{verbatim}
    
  Using~Algorithm~\ref{alg:find-manipulation}, we managed to find the following manipulation for student 134:
  \begin{verbatim}
    [(8, 360.0), 
     (23, 6.30), (29, 5.10), (34, 1.95), (19, 1.35), 
     (33, 0.1125), 
     (4, 0.0060), (7, 0.0045), (3, 0.0030)]
  \end{verbatim}
  The only difference between this manipulation and the original profile is that weights of course 8 and 23 are swapped.
  We then compute the distribution of the utility from reporting these two utility profiles and compare them in the following figure, where $\mathcal{D}_{134}$ is the utility distribution from reporting truthfully, and $\mathcal{D}_{134}'$ is the utility distribution from reporting the manipulation.

    \begin{figure}[H]
    \centering
    \includegraphics[scale=0.6]{img_case_studies/SP_s3-tuck-fall-2020-5-additive.in_0.0005_0.01_5000_5_2_1_1_1_dbatch-1_ebatch-1_fullstepsizes_util-log.pickle.pdf}
  \end{figure}  
\Qianfan{
  $p=2.3\times 10^{-11}.$ It seems that the increase is small. But it is not a negligible manipulation because it will NEVER harm the utility, as we can see from the case study below.}

How does the manipulation work? \Qianfan{TBD}
% In a nutshell, Student 134 manipulate their report to claim that their default allocation is unacceptable to them (specifically, it causes them to envy a lower-ranked student). This forces the algorithm to give them a better allocation in order to satisfy the EF-TB constraint. We now look into the detail. 

\paragraph{Simplifications}
  
  To simplify the analysis of the case study, we make the following two small tweaks to the real results (the real results are qualitatively very similar):
  Specifically, we focus on a manipulation by Student 134, and we also consider the possible allocations for Student 184 and 234 since their allocations are tightly related to student 134's manipulation.
  
  \begin{enumerate}
      
  \item Though the manipulation improves Student 134's utility in expectation, we fix a realization of initial budgets $\vc{b_0}$ for the case study and see how it helps Student 134. As noted above, even when we resample the initial budgets the gain from the manipulation is statistically significant; but keeping the initial budgets fixed will help keep the analysis tractable.
  
  \item   Note that in the manipulated case, Algorithm~\ref{alg:tatonnement} will return some different market-clearing price $\vc{p'}$ than the original on $\vc{p^*}$, but the difference between $\vc{p^*}$ and $\vc{p'}$ is tiny and the manipulation still works if we can only run a budget perturbation process under price $\vc{p^*}$. Thus, we assume the price is always $\vc{p^*}$ in the case study, and we focus on the budget perturbation process only.
  
  \item 
  The following analysis is a local one, in the sense that we treat other students' allocations as fixed in the budget perturbation process for simplicity (they are actually not fixed in practice).
  \end{enumerate}
  
\paragraph{Prices \& capacities:} 
Since we treat other students' allocations as fixed, we can calculate each courses' remaining capacities for these three students. And we use $\ast$ to denote unimportant courses (i.e., courses do not occur in possible allocations).
\begin{table}[H]
\centering
\begin{tabular}{|c|c|c|c|}
\hline
 Relevant courses  & {\bf 8} & {\bf 29} & others    \\ \hline
Market-clearing price $\vc{p^*}$ & 10200  & 170  & 0 \\ \hline
Remaining capacity (locally) & 2 & 1 & $>1$ \\ \hline
\end{tabular}
\end{table}

\paragraph{Preferences, budgets, and possible allocations (irrelevant courses omitted):}
In the table below we describe the budgets and preferences of the relevant students.
For example, when we set $b^*_{134}=b_{0,134}-75=10199$, student 134's allocation $a_{134}(\vc{u},\vc{c},\vc{p}^*,\vc{b}^*)$ will be the bundle $[23, {\bf 29}, 34, 19, 33]$, since she cannot afford course ${\bf 8}$.

Note that in this case, even after student 134's manipulation, her possible allocations remain unchanged. However, the final allocation that Algorithm~\ref{alg:tatonnement} made will be different due to different EF-TB constraints.
    \begin{table}[H]
    \centering
    \begin{tabular}{|c|c|c|l|}
    \hline
                & Preferences                                                         & Initial budget $\vc{b_0}$ & Possible (allocation, perturbation)\\ \hline
    Student 134  & $23 \gg {\bf 8} > {\bf 29} > 34 > 19 \gg 33 > \ast$                                                & 10274          & \begin{tabular}[c]{@{}l@{}} 
    ($[23, {\bf 29}, 34, 19, 33]$, $-75$)\\ ($[23, {\bf 8}, 34, 19, 33]$, $0$)\\ ($[23, {\bf 8}, {\bf 29}, 34, 19]$, $+96$) \end{tabular}\\ \hline
    \begin{tabular}[c]{@{}c@{}}\textbf{Student 134'}\\ (manipulated)\end{tabular} & $ {\bf 8} \gg 23 > {\bf 29} > 34 > 19 \gg 33 > \ast$   & 10274          & \begin{tabular}[c]{@{}l@{}} 
    ($[23, {\bf 29}, 34, 19, 33]$, $-75$)\\ ($[23, {\bf 8}, 34, 19, 33]$, $0$)\\ ($[23, {\bf 8}, {\bf 29}, 34, 19]$, $+96$) \end{tabular} \\ \hline
    Student 184  & ${\bf 8} \gg 22 \gg 23 > {\bf 29} \gg 38 > 0 > \ast$                                                  & 10264  & \begin{tabular}[c]{@{}l@{}} ($[22,23,{\bf 29},38,0]$, $-65$) \\ ($[{\bf 8}, 22, 23, 38, 0]$, $0$) \end{tabular}        \\ \hline
    Student 234  & $19 \gg {\bf 8} > 25 > 38 \gg 17 > 13 > \ast$                                                  & 10220  & \begin{tabular}[c]{@{}l@{}} ($[19, 25, 38, 17, 13]$, $-21$) \\ ($[19, {\bf 8}, 25, 38, 17]$, $0$) \end{tabular}        \\ \hline
    \end{tabular}
    \end{table}

    Also note that we only includes those allocations with budget perturbation not greater than $100$ in the table above, which is determined by the $\epsilon$ parameter of Algorithm~\ref{alg:tatonnement}.

% There are two other important students whose preferences and allocations are not described in the above table (for simplicity), and treated as fixed for our case study analysis. In particular all the allocations we consider, both of these students receive Course 8 (as well as other courses)% \footnote{Why doesn't the algorithm force them to give up course 8 by budget perturbation? When these students drop Course 8, they try to get other full courses (2, 29 respectively). Forcing them to also drop Courses 2 and 29 requires a larger budget perturbation (in terms of $\|\vc{b}^*-\vc{b_0}\|_1$), which would force changes to other students', etc.}. These students (numbered 99, 163) have lower initial budgets than Student 71. Although their allocation is fixed, they impact the algorithm's output because they enforce an envy constraint on Student 71- to satisfy EF-TB,  71 cannot be allocated a less-preferred bundle because its initial budget is higher. 



\paragraph{Possible market-clearing allocations:}
In the following, we present possible market-clearing allocations under different reported preferences.

\begin{table}[H]
\centering
\begin{tabular}{|l|c|l|}
\hline
\multicolumn{1}{|c|}{Allocation}                                                                 & $\|\vc{b}^*-\vc{b_0}\|_1$ & \multicolumn{1}{|c|}{Comments}   \\ \hline
\begin{tabular}[c]{@{}l@{}}134: $[23, {\bf 29}, 34, 19, 33]$    \\  184: $[{\bf 8}, 22, 23, 38,0]$  \\ 234: $[19, {\bf 8}, 25, 38, 17]$\end{tabular}  & $75+0+0=75$ &
\begin{tabular}[c]{@{}l@{}}Chosen in the original case due to smaller l1 norm\\ No longer available in the manipulated case,\\ since now student 134 will envy student 184 \end{tabular}  \\ \hline
\begin{tabular}[c]{@{}l@{}}134: $[23, {\bf 8}, {\bf 29}, 34, 19]$   \\  184: $[{\bf 8}, 22, 23, 38,0]$  \\ 234: $[19, 25, 38, 17, 13]$\end{tabular}  & $96+0+21=117$  &  Chosen in the deviated case \\ \hline
\begin{tabular}[c]{@{}l@{}}134: $[23, {\bf 8}, 34, 19, 33]$ \\ 184: $[22,23,{\bf 29},38,0]$ \\ 234: $[19, {\bf 8}, 25, 38, 17]$ \end{tabular} & $0+65+0=65$     & \begin{tabular}[c]{@{}l@{}}Invalid in both cases since student 184 envys student 234
\end{tabular}  \\ \hline
\end{tabular}
\end{table}

As a result of the manipulation, Student 134 gets course 8 instead of 33, a huge improvement.

\paragraph{Cmments:}
\Qianfan{TBD}
% It seems that the manipulation is extremely simple (not reporting course 1) and successfully fooled EF-TB constraints.
% However, further experiments suggests that it fails to generalize to both following scenarios:
% \begin{itemize}
%     \item It is no longer profitable to Student 71 under the resampled population setting.
%     \item It is not profitable to any other Student under the same setting, i.e., resampled randomness.
% \end{itemize}
% In the next section, we will see that without EF-TB constraints, we can find much more powerful manipulations in the sense that it can generalize to both cases well.
% \Qianfan{However, this holds for this specific dataset, which is somewhat limited because 1) it's 5-additive, 2) it has a strange structure of utility profile.}



\subsection{strong EF-TB constraints case study}

\paragraph{The manipulation}

We are now looking at student 4. The raw data from student 4's utility is as follows, where each tuple $(c_i,w_i)$ indicates her weight for course $c_i$ is $w_i$.
\begin{verbatim}
[(8, 360.0), 
 (25, 6.42), (23, 5.88), (26, 4.80), (19, 3.48), (27, 2.67), (6, 2.1), (37, 1.83), 
 (3, 1.56), (33, 1.29), (20, 1.02),
 (34, 0.1575), (36, 0.1275), (7, 0.0975), (21, 0.0675), 
 (39, 0.0090)]
\end{verbatim}

The manipulation we found is as simple as report course 39 as the second favourite course, i.e.,
\begin{verbatim}
[(8, 360.0), 
 (39, 10.00), (25, 6.42), (23, 5.88), (26, 4.80), (19, 3.48), (27, 2.67), (6, 2.1), (37, 1.83),
 (3, 1.56), (33, 1.29), (20, 1.02),
 (34, 0.1575), (36, 0.1275), (7, 0.0975), (21, 0.0675)]
\end{verbatim}

\Qianfan{TBD- explain how the manipulation works}

In the following analysis, we still make same simplifications to the last section, i.e., fixing a realization for initial budgets and do a local analysis.

\paragraph{Prices \& capacities} 
    The following table contains the prices and capacities of relevant courses.
    \begin{table}[H]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
     Relevant courses & {\bf 8}  & {\bf 39} & others    \\ \hline
    Market-clearing price $\vc{p^*}$ & 10160 & 10 & 0 \\ \hline
    Remaining capacity (locally) & 1 & 1 & $>1$ \\ \hline
    \end{tabular}
    \end{table}

   \paragraph{Preferences, budgets, and possible allocations:}
    In the table below we describe the budgets and preferences of the relevant students.
  
    \begin{table}[H]
    \centering
    \begin{tabular}{|c|c|c|l|}
    \hline
                & Preferences                                                         & Initial budget $\vc{b_0}$ & Possible (allocation, perturbation)\\ \hline
    Student 4  & ${\bf 8} \gg 25 > 23 > 26 > 19 > 27 > \ast \gg {\bf 39}$                                                & 10211          & \begin{tabular}[c]{@{}l@{}} 
    ($[25, 23, 26, 19, 27]$, $-52$)\\ ($[{\bf 8}, 25, 23, 26, 19]$, $0$) \end{tabular}\\ \hline
    \begin{tabular}[c]{@{}c@{}}\textbf{Student 4'}\\ (manipulated)\end{tabular} & ${\bf 8} \gg {\bf 39} > 25 > 23 > 26 > 19 > 27 > \ast$                                                & 10211          & \begin{tabular}[c]{@{}l@{}} 
    ($[{\bf 39}, 25, 23, 26, 19]$, $-52$)\\ ($[{\bf 8}, 25, 23, 26, 19]$, $-42$) \\ ($[{\bf 8}, {\bf 39}, 25, 23, 26]$, $0$) \end{tabular}\\ \hline
    Student 193  & \begin{tabular}[c]{@{}c@{}}${\bf 39} \gg {\bf 8} > 22 >10 \gg 18 > 17 > \ast$\end{tabular}                                                   & 10255  & \begin{tabular}[c]{@{}l@{}} ($[{\bf 39}, 22, 10, 18, 17]$, $-86$) \\ ($[{\bf 39}, {\bf 8}, 22, 10, 18]$, $0$) \end{tabular}        \\ \hline
    \end{tabular}
    \end{table}
    
 \paragraph{Possible market-clearing allocations:}
  In the table below we present possible market-clearing allocations under different reported preferences.
  
    \begin{table}[H]
    \centering
    \begin{tabular}{|l|c|l|}
    \hline
    \multicolumn{1}{|c|}{Allocation}                                                                 & $\|\vc{b}^*-\vc{b_0}\|_1$ & \multicolumn{1}{|c|}{Comments}   \\ \hline
    \begin{tabular}[c]{@{}l@{}}4: $[25, 23, 26, 19, 27]$    \\ 193: $[{\bf 39}, {\bf 8}, 22, 10, 18]$\end{tabular} & $52+0=52$  &
    \begin{tabular}[c]{@{}l@{}}Chosen in the original case due to smaller l1 norm\\ No longer available in the deviated case \end{tabular}  \\ \hline
    \begin{tabular}[c]{@{}l@{}}4: $[{\bf 8}, 25, 23, 26, 19]$    \\ 193: $[{\bf 39}, 22, 10, 18, 17]$\end{tabular} & $42+86=128$ & Chosen in the manipulated case \\ \hline
    \end{tabular}
    \end{table}
    
    As a result of the manipulation, Student 4 gets course 8 instead of 27.






% \paragraph{Generalizing the manipulation}

% We try to generalize the manipulation to those students who originally do not want course 2 at all. Specifically, the manipulation for these student is by simply adding a $(2, 10.00)$ pair to the utility profile, which always makes course 2 the second favourite by the special structure of utility profile.
% \Qianfan{For those students actually want course 2 (like student 76), I think the manipulation would work as well, but we should verify it.}


% Under the resampled randomness setting, the result is as follows (where we use 200 samples to compute the expected profit for each student):

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{img/SP_s3-tuck-fall-2020-5-additive.in_0_300_0.0005_0.01_200_10_2_1_0_False_0.0_equalbudgets_uniquesol_deviation17937_noEFTB.pickle_as_a_whole.pdf}
% \end{figure}

% The result shows that the manipulation remains profitable for many students. And for those students who do not benefit from the manipulation, they would not loss too much either, which makes the manipulation very powerful.

% Furthermore, under the resampled population setting, we also observed something similar. The result is as follows \Qianfan{where we still use 200 samples to get the expected profit -- might be too small for this setting}

% \begin{figure}[H]
% \centering
% \includegraphics[width=0.7\textwidth]{img/SP_s3-tuck-fall-2020-5-additive.in_0_300_0.00025_0.01_200_10_2_2_0_False_0.0_equalbudgets_uniquesol_deviation17937_noEFTB.pickle_as_a_whole.pdf}
% \end{figure}

% \Qianfan{The result is inaccurate because we selected only a subset of students (125 of 194) due to a bug in the code. But the conclusion should remain same when we fixed it.}

% \paragraph{Similar manipulations}

% One natural question is that: how about similar manipulations?
% It seems that what the manipulation did is to reporting a course with small price as the second favourite course.
% Therefore, we tested whether this kind of manipulations work with course 1 6, 29, 39 (courses that usually end up with a small non-zero price).
% Some of them work, yet others not.
% Following are the results in the resampled randomness setting:

% % \Qianfan{
% % All non-zero prices are as follows:
% % }
% % \begin{verbatim}
% % [(1, 0.001), (2, 0.0005), (6, 0.0725), (8, 1.0195), (29, 0.0425), (32, 1.0195), (39, 0.0015)]
% % \end{verbatim}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{img/SP_s3-tuck-fall-2020-5-additive.in_0_300_0.0005_0.01_200_10_2_1_0_False_0.0_equalbudgets_uniquesol_deviation17936_noEFTB.pickle_as_a_whole.pdf}
% \end{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{img/SP_s3-tuck-fall-2020-5-additive.in_0_300_0.0005_0.01_200_10_2_1_0_False_0.0_equalbudgets_uniquesol_deviation17940_noEFTB.pickle_as_a_whole.pdf}
% \end{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{img/SP_s3-tuck-fall-2020-5-additive.in_0_300_0.0005_0.01_200_10_2_1_0_False_0.0_equalbudgets_uniquesol_deviation17965_noEFTB.pickle_as_a_whole.pdf}
% \end{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{img/SP_s3-tuck-fall-2020-5-additive.in_0_300_0.0005_0.01_200_10_2_1_0_False_0.0_equalbudgets_uniquesol_deviation17963_noEFTB.pickle_as_a_whole.pdf}
% \end{figure}



% \section{Comparison between EF-TB constraints (preliminary)}

% With the observations from the previous two sections, it seems interesting to compare the distributions of profitable manipulations with or without EF-TB constraints.
% Still, the experiment is performed on the 5-additive instance.
% And we also add a restricted version EF-TB called \emph{restrict EF-TB}, where EF-TB constraints are restricted to courses with weight $\ge 1$.

% In the experiment, Algorithm~\ref{alg:find-manipulation} with 10 samples is used to find manipulations, and we further use 200 samples to evaluate the expected profit for each manipulation.
% Note that not all manipulations found are profitable (with respect to the 200 samples), and we only keep profitable ones.

% The comparison of total numbers is as follows:

% \begin{table}[H]
% \centering
% \begin{tabular}{|c|c|c|c|}
% \hline
%   & Full EF-TB  & Restricted EF-TB & No ET-TB    \\ \hline
% \# of profitable manipulations & 35 & 33 & 37 \\ \hline
% Average expected profit & 1.68 & 1.58 & 24.07\\ \hline
% Maximum expected profit & 14.25 & 10.19 & 110.38\\ \hline
% \end{tabular}
% \end{table}

% We also plot the actual distributions of the expected gain in the following figures:
    
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{img/5-additive-with-full-EFTB-overall.pdf}
% \end{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{img/5-additive-with-restricted-EFTB-1000-overall.pdf}
% \end{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.5\textwidth]{img/5-additive-without-EFTB-overall.pdf}
% \end{figure}

% From these results, one can see that:
% \begin{itemize}
%     \item the number of profitable manipulations are quite close in all three cases;
%     \item however, the expected profit will be much higher in the case without EF-TB constraints.
% \end{itemize}

% % testddd
% % Say the student's utility is something like a >> b,c,d,e
% % a >> 2 >> b,c,d,e
% % Originally:  initial budget B0 < p_a, price p_a           B0 >= p_a
% % #1: not allocating a:  0                                  B0-p_a
% % #2: allocate a:        p_a-B0                              0

% % Deviated:  
% % #1 not allocating a:   0                                    B0-p_a
% % #2 allocate a:         p_a-B0                               0

% \iffalse
% \begin{enumerate}
%     \item The additive case:
%     \begin{enumerate}
%         \item Without any constraints (i.e., purely additive), no profitable manipulation can be found using the method above.
%         \begin{itemize}
%             \item Reason?
%         \end{itemize}
%         \item With a single constraint that every student can take at most 5 courses, there's still some profitable manipulations.
%         \begin{itemize}
%             \item Case study shows that the manipulation are through effect on budget perturbation.
%             \item It seems that EF-TB constraints are too weak, hence there will be a lot of possible optimal perturbations, some of them in favor of the student $i$, some of them not. 
%         \end{itemize}
%     \end{enumerate}
%     \item Freezing the budget:
%     \begin{enumerate}
%         \item It turns out that no profitable manipulation can be found if we freeze the final budget $b_i^*$ in the perturbation (which is also an evidence that previous manipulations are through effect on budget perturbation).
%         \item A quick fix: in the beginning of our algorithm, randomly choose some students (say, $50\%$) and always fix their budgets. 
%     \end{enumerate}
% \end{enumerate}
% \fi





\Aviad{Do we need to keep any of the following? I moved the 5-additive discussion to Case Study section \texttt{original}: An original instance including 40 courses and 283 students from a business school, where Each student's utility function is defined using
    \begin{itemize}
        \item A weight $w_j$ for each course $j$.
        \item A list of possible conflicts, where each conflict contains a subset of courses $S$ and a threshold $T$ indicating either
        \begin{itemize}
            \item the student can only take at most $T$ courses in $S$, or
            \item the student can only take at most $T$ academic credits in $S$.
        \end{itemize}
        All conflicts must be satisfied, i.e., the bundle violating any of the conflicts will be considered as invalid for the student.
        \item A list of requirements, where each requirement contains a subset of courses $S$ and a threshold $T$ indicating either
        \begin{itemize}
            \item the student should take at least $T$ courses in $S$, or
            \item the student should take at least $T$ academic credits in $S$.
        \end{itemize}
        If all requirements cannot be satisfied simultaneously, then the student will seek to maximize the number of satisfied requirements as the first priority.
    \end{itemize}
    And the utility function can be defined in the aforementioned way via a tuple $(\vc{w},valid,req)$ where $\vc{w}=(w_j)_{j\in [m]}$, and for every bundle $\vc{x}\in 2^{[m]}$,
    \begin{align*}
        valid(\vc{x})&=\begin{cases}1 & \text{bundle $\vc{x}$ satisfies all conflicts}\\0 & \text{otherwise}\end{cases}\\
        req(\vc{x})&=(\text{number of satisfied requirements with bundle $\vc{x}$})
    \end{align*}
  %  \item \texttt{5-additive}: The 5-additive version of the above instance, i.e., ignoring all conflicts and requirements, except for a single constraint that every student can take at most 5 courses. 
 %   \item \sout{\texttt{purely-additive}: The additive version of the above instance, i.e., removing all the validity constraints and requirements (letting all $valid(\vc{x})=1, req(\vc{x})=0$).} \Aviad{Currently not implemented because it makes the algorithm too slow.}
    
%\end{enumerate}

Among these instances, the weight of a student's favourite course lies in the range between $180$ to $360$ mostly. And the minimum non-zero weight can be as small as $ 10^{-3}$.}





\section{Future Directions}



It is known that, in general settings, tatonnement need not converge to an equilibrium.
\Aviad{[ABE COMMENT FOR THEORISTS]: Informally, this is because finding market equilibria is PPAD and so if tatonnement worked then you could  easily solve PPAD. Please help to make this argument rigorous and-or cite the appropriate resources, thanks!}
However, our results imply that continued application of tatonnement is able to ``power through" local maxima to find excellent approximate equilibria with very low clearing error. This suggests that the relationship between prices and demand for the course allocation problem---and potentially other problems of economic interest with complex agent preferences and heterogeneous goods---may be much simpler than has been previously believed and may be far more tractable in practice than their worst-case theoretical bounds. Recalling Jain's dictum, perhaps many more market equilibria can be found by laptops---or, perhaps, Walras's seemingly naive description of how prices iterate in the real world may generally produce approximate equilibria in practice.
% Abe note: this result is actually broadly in line with some current findings, like at https://arxiv.org/abs/1908.00844 but nobody has the "real" utility functions to back them up
Along these lines, there has been some recent work on improving bounds for gradient-descent-type algorithms for market equilibria [CITE COLE PAPERS]. 

The idea of trying to figure out ways to ``power up" gradient descent to find global minima in an apparently complex but potentially well-formed multidimensional space draws us to a surprising parallel with an area of research that has seen an explosion of activity in the past decade: deep learning. We plan to explore whether adding some of the techniques that have improved iterative gradient descent in deep learning, like momentum, could also provide a speedup for our heuristic algorithm in price space.

Something about how the algorithm is fast enough now to do experiments.

==> old-intro.tex <==

Competitive Equilibrium from Equal Incomes (CEEI)~\cite{Fol67,Var74,TV85} is an attempt to leverage the efficiency of market equilibria while preserving the \emph{ex post} fairness properties that come from equal incomes.
%
For complex preferences, however, CEEI does not necessarily exist.

Budish~\cite{Budish2011} developed a modification of CEEI, Approximate CEEI (A-CEEI). He showed that an approximate equilibrium from approximately equal incomes always exists.

\Aviad{Abe would like you to add some stuff about SP-L and EF-TB here}

Budish's original theoretical work used a fixed-point theorem and is inherently non-constructive. It was shown in~\cite{OthmanPR16} that finding an A-CEEI is \PPAD-complete. This is similar to many other economic equilibria whose existence rely on non-constructive proofs, the most famous of which is the Nash equilibrium~\cite{DaskalakisGP09,ChenDT09}. 

Despite this theoretical infeasibility, a heuristic algorithm exists that solves the problem adequately in practice~\cite{BudishCKO17}. This algorithm uses local search to progressively refine the prices assigned to courses. Local search is embarrassingly parallel and in practice that algorithm is run over many search starts on many compute servers.

The existing heuristic algorithm makes A-CEEI a practical solution concept for settings that require efficiency and fairness but for which the use of real money is impractical or repugnant. The setting  where A-CEEI has seen the most practical application is in the allocation of courses to students.
%
 Student preferences are often quite complex in course allocation. Students often demand several courses and individual courses could be complements or substitutes depending on the bundle of other courses in a student's schedule. Course allocation---particularly in professional schools---also tends to be a challenging allocation problem, as the most popular ``star courses" tend to have far more demand than supply.
%
We explore the course allocation problem experimentally in this paper using real student preferences over real professional school courses.


While the existing heuristic algorithm is able to solve a \PPAD-complete problem in practice, it introduces some additional potential manipulability. The heuristic algorithm is a three-stage process. The first stage finds an approximate equilibrium, which equilibrium will tend to have both undersubscription in positive-price courses as well as oversubscription. The second stage progressively increases course prices, to eliminate all oversubscription. The final stage is a ``backfill" process, where students are sequentially allocated extra budget and allowed to spend that budget on courses that are undersubscribed.

While the backfill process substantially reduces the deadweight loss of computed assignments it may have problematic incentive and fairness properties. Students who get first shot at spending that extra budget in the backfill may be able to add an excellent course to their schedule. This backfill process is only necessary because of the clearing error found in the original approximate equilibrium, and it motivates the search for a better solver; an algorithmic technique that consistently produced zero-clearing-error solutions would have nothing to backfill. 

\Aviad{How should we call the different EF-TB constraints? Regular and Strong? Classic and Robust? Other suggestions?}

\Aviad{To do throughout the paper, especially Case Studies section: anonymize / remove school names, etc}

\subsection{Contribution I: A (much) faster heuristic algorithm for computing A-CEEI}
Our first contribution is an improved heuristic algorithm for computing A-CEEI. Our algorithm outperforms the commercial state-of-the-art by several orders of magnitude in both the quality of produced solution as well as runtime on real course allocation problems.

Kamal Jain's famous formulation ``if your laptop cannot find it then neither can the market" [CITE: AGT Book. I can't actually find this quote anywhere in a paper?]
 was originally intended as a negative result, casting doubt on the practical implications of many famous economic concepts because of their worst-case computational complexity results. Even for course allocation, where a heuristic algorithm exists and seems to work in practice, Jain's formulation seemed to still bind, as solving A-CEEI involved an intense day-long process with a fleet of high-powered cloud servers operating in parallel.
%
The work detailed in this paper has significantly progressed what laptops can now find: even the largest and most challenging real course allocation problems we have access to can now be solved in a few hours on a commodity laptop.


%\footnote{To be precise we improve over the {\em previous} commercial state-of-the-art --- a variant of the algorithm we developed in this work is now deployed by Cognomos.} on all fronts, sometimes by multiple orders of magnitude, see e.g.~Figure~\ref{fig:TBD} \Aviad{TBD: move figure to intro }.
% Abe doesn't think this is a good idea. No figures in the Intro, don't even really need the forward pointer.

We highlight some of our algorithmic findings here, with details in Sections~\ref{sec:algo} and \ref{sec:perform}. Further details about the previous state-of-the-art algorithm (henceforth {\em benchmark}), can also be found in academic publications~\cite{OthmanSB10, BudishCKO17}. 
At a high level, both our algorithm and the benchmark, perform variants of the classic tatonnement algorithm: increase the price of over-demanded courses, and decrease the prices of under-demanded courses.

One of the main technical innovations introduced in the benchmark algorithm was the use of individual price adjustments: on some iterations, the algorithm can make a larger improvement on the clearing error by adjusting the price of a single course rather than all the courses simultaneously. Based on extensive experiments on randomly generated data (real data from students bidding was not yet available at the time),~\cite{OthmanSB10} reported that the algorithm was much more likely to find a solution with acceptable clearing error when mixing individual price adjustments and full tatonnement updates. 
Our first algorithmic insight is to largely {\em reverse this finding of~\cite{OthmanSB10}}. We observe that on real world instances it is in fact much more efficient to use only full tatonnement updates, even when they locally increase the clearing error. We discuss evidence, explanations, and caveats of  this finding in Section~\ref{sec:perform}.


Our second (and perhaps more interesting) algorithmic insight focuses on the ``end game'', when the algorithm is already close to a reasonable clearing error. Here, we show that making tiny-but-cleverly-optimized perturbations to the {\em budgets} (rather than prices) can quickly lead to the holy grail of zero clearing error. Before going into the details, we remark that (i) in the practical benchmark implementation, students budgets are already perturbed at random (and with larger perturbations); (ii) our insight  is inspired directly by the non-algorithmic existence proof in~\cite{Budish2011}, which perturbs the students' budgets twice: once to guarantee a desirable fixed point of the tatonnement correspondence, and a second time to break ties between marginal students at the fixed point. 

To describe the budget perturbations, let's start from the end: we would like to return a vector of course prices and almost-equal student budgets and (ideally) zero clearing error. Towards this, at each iteration of the tatonnement the algorithm checks solves an (NP-hard but fast in practice) integer program to look for a small budgets perturbation that will nudge students' demand bundles to zero the overall market clearing error. More generally, at each iteration we can find the {\em optimal budgets perturbation}, aka the one that minimizes the clearing error. Since our ultimate goal is to find a price vector that works well with an optimal budget perturbation, we use the clearing error with respect to the optimal budget perturbation to perform the next iteration of tatonnement.

While the idea of using optimal budget perturbations is extremely effective algorithmically, we have to be careful not to open opportunities for manipulability: although budget increases are very small, doing it based on student's reported course preferences could open an opportunity for strategic reporting. To this end, we encode in our integer program the same EF-TB constraints, that guarantee the SP-L (Strategyproof in the Large) condition for the original A-CEEI mechanism. Although this makes the integer program larger, we can solve it very efficiently (see Section~\ref{sub:fast-EF-TB} for some optimizations). 


\begin{figure}[t]
\centering
\includegraphics[width=.66\textwidth]{img_errors/s3-toronto-law-fall-19-robustL-errors-wrt-time.pdf}
\caption{Clearing errors of the algorithms with respect to the running time (based on 4-hour runs).}
\label{fig:progress-of-algos-error-4h}
\end{figure}


%TBD: discuss the new algorithm and comparisons with previous algorithm, other approaches.

\subsection{Contribution II: Empirically evaluating the incentives of A-CEEI}

In theory, the A-CEEI mechanism has a very desirable property: it is {\em Strategyproof in the Large (SP-L)}; i.e.~the expected utility any student can gain by misreporting their true preferences diminishes as the number of students goes to infinity~\cite{AB18}. What does this theory guarantee for realistic schools with a finite number of students? 
Unfortunately, the answer is not much: the SP-L theoretical guarantee only starts kicking in when the number of students is much larger than the number of possible types. For the general A-CEEI mechanism%
\footnote{In practice, students' reporting language is often more restricted, but still the number of students is always much smaller than the number of possible types.}, a type consists of a ranking of all possible schedules; the number of possible schedules is exponential in the number of courses, and the number of ways they can be ranked adds another layer of exponentiation. In other words, until the number of students is {\em doubly-exponential} in the number of courses, the theoretical guarantee of SP-L is meaningless. 

The situation is further complicated by the computational intractability of the A-CEEI problem. 
A natural approach for dealing with the large number of possible deviations is to directly analyze the way students could manipulate the algorithm's choice of equilibrium. This has been fruitful in analyzing simple algorithms~\cite{Vitercik21-thesis,AKLLM20}. But because of the \PPAD-hardness of the A-CEEI problem we resort to a highly nontrivial heuristic algorithm  (see Contribution I). Theoretically analyzing how a possible misreport of preferences would affect the trajectory in price space taken by this algorithm seems far from tractable.

Going beyond intractable theoretical guarantees on students' incentives, our approach is to empirically evaluate them. 
Our main question in this part is:
\begin{quote}
    In practice, can students gain in the A-CEEI mechanism by manipulating their reported preferences?
\end{quote}


Here, it is paramount that we have our novel fast heuristic algorithm: Previously, it was barely possible to compute one allocation, so re-computing allocations for each possible deviation was completely out of the question. Anecdotally, this is the reason why the computational exploration of the same issue in Budish's original paper was limited to  tiny examples with 2 students and 4 courses~\cite[Footnote 31]{Budish2011-old}.

Still, no matter how fast our equilibrium computation algorithm, we cannot possibly enumerate all possible deviations (again, in theory their number is doubly exponential in the number of courses). However, it is reasonable to expect that computationally- and informationally-bounded students also cannot test every possible deviation. We thus model a strategic student using a simple hill-climbing algorithm that adjusts the single course weights starting from the original truthful report. We also consider different restrictions on the student's information about the market, as detailed in Definition~\ref{def:manipulation}.

In Section~\ref{sec:manip} We use our manipulation-finding algorithm in combination with our fast A-CEEI finding algorithm to explore the plausibility of effective manipulations for students bidding in A-CEEI. Originally, we had expected that since our mechanism satisfies the EF-TB and SP-L properties, it would at least be practically strategyproof --- if even we don't really understand the way our algorithm chooses among the many possible equilibria, how can a student with limited information learn to strategically bid in such a complex environment?

Surprisingly, we stumbled upon a simple and effective manipulation for (the first iteration of) our mechanism. We emphasize that although the manipulation is simple in hindsight, in over a year of working on this project we failed to predict it by analyzing the algorithm --- {\em the manipulation was discovered by the algorithm}. 

Inspired by this manipulation, we propose a natural strengthening of EF-TB. We encode this {\em robust EF-TB} as a new constraint in our algorithm (specifically, the integer program for finding optimal budget perturbations). Fortunately, our algorithm is still very fast even with this more elaborate constraint. And, when we re-run our manipulation-finding experiments, we observe that robust EF-TB significantly reduces the potential for manipulations in practice.



\subsection{Robust Envy-Free-with-Tie-Breaking}
In this section we gradually build towards our new notion of robust EF-TB.
We begin with the classical notion of {\em Envy-Free (EF)}: an allocation is said to be envy free if no student $i$ prefers the schedule allocated to another student $i'$. 

In the course allocation problem, due to the challenges of integrality constraint and combinatorial demand, EF allocations rarely exist. 
Azevedo and Budish~\cite{AB18} relax the notion of EF to allow {\em tie-breaking} (EF-TB): The students are ranked at random%
\footnote{In practice a combination of seniority and random ranking may be used.}, and the allocation is said to satisfy EF-TB if no student $i$ envies any lower-ranked students. (However, $i$ may envy higher-ranked students.)
EF-TB is not a very satisfying fairness criterion%
\footnote{For fairness,~\cite{Budish2011} introduced the notion of Envy-Free-up-to-1-good (EF1) and proved that it is satisfied by A-CEEI.}, but it does imply strategyproof-in-the-large (SP-L)~\cite{AB18}. 

A-CEEI allocations satisfy EF-TB when the budgets are assigned at random because no student can envy another student with a lower budget (if $i'$'s budget is lower, then $i'$'s schedule must also be affordable for $i$). When we introduce optimal budget perturbations, we simply encode  EF-TB as a constraint in our perturbation-finding integer program. While in theory this approach satisfies SP-L, in practice it can open the door to manipulations, as described in the following example.

\subsubsection{Surprisingly simple manipulations}

We henceforth refer to the EF-TB criterion as {\em classic EF-TB} to distinguish it from the upcoming robust EF-TB. 

\begin{example}[Manipulation with classic EF-TB constraints]\label{ex:regular-manipulation} \hfill

Alice and Bob both want the last seat in the popular CS161 course. But Alice is even more excited about taking independent research units with her advisor (of which there is unlimited supply, so the price is always zero); she would like to take both. Bob's second choice is  ECON101, which is already full.

Even if Alice ranks higher, the algorithm attempts to perturb her budget below Bob's --- otherwise Bob has to be assigned a seat in the full ECON101, causing a clearing error. 
If Alice reports her true preferences, she will not envy Bob because she still has her independent research units. But if she ranks independent research units lower than CS161, she would envy Bob whenever he gets the last seat to CS161. Hence by deviating, Alice strictly increases her chances of also getting into CS161. 

Note that ranking the free course (independent research units) lower {\em never hurts} Alice. 
So this manipulation is profitable in expectation for Alice even if she only has very noisy information about her rank and other students' demand. 
\end{example}

Interestingly, this manipulation works {\em because} of the EF-TB constraints that we introduce to prevent manipulations! In Section~\ref{sec:case-study} we also describe a simple manipulation that works when EF-TB constraints are not enforced. 

We also describe a third manipulation (Example~\ref{TBD}) which unfortunately works with all variants of our algorithm, including robust EF-TB constraints. We conjecture that it also works with the original A-CEEI algorithm; however, that algorithm is prohibitively slow so it is hard to test this conjecture. Either way, our numerical experiments suggest that this manipulation is unlikely to be very effective for most students. 

All three examples of manipulations share the feature that they are robust; in particular the manipulating student risks very little by applying them, even if they have limited information about the market. We also highlight that although we present simplified examples with fake names and course numbers, all three examples are directly based on manipulations discovered by our algorithm in almost-real%
\footnote{In our experience it is very hard for humans to understand the algorithm's choice of manipulations in real instances because students' demand function is very complicated. For the purpose of extracting interpretable manipulations, we took the true reported course weights, but replaced the complicated feasibility constraints by a best-schedule-of-5-courses constraint.}
 instances.

\subsubsection{Introducing robust EF-TB}

Our notion of robust EF-TB is directly motivated by Example~\ref{ex:regular-manipulation}.
Arguably, in this example it is most natural not to count Alice's independent research units when estimating her envy towards Bob. 

Of course, we don't know which class number corresponds to ``independent research units'' --- but more generally we don't want to count any free%
\footnote{In the context of A-CEEI it makes sense to define {\em free} with respect to the equilibrium prices. For a general mechanism, we can say that a course is ``free'' if it is undersubscribed, yet no student who would rather add it to their schedule.}
courses for the purpose of robust EF-TB. In more detail (see Section~\ref{sec:prelim} for formal definitions), we say that Alice {\em robust-envies} Bob if she prefers any subset of $\{\text{Bob's schedule}\} \cup \{\text{free courses}\}$ over her own allocation. We say that a mechanism is {\em robust EF-TB} if it always produces assignments such that no higher-ranked student  robust-envies any lower ranked student. 

Note that robust EF-TB is a strengthening of EF-TB. Observe also that if all the budgets respect the random TB rule, then any A-CEEI allocation is robust EF-TB. In our algorithm, because of the optimal budget perturbations, the budgets in our algorithm may not respect the original TB order; instead, we encode the robust EF-TB constraint in the integer program that optimizes over budget perturbations.  






%* Define EF-TB
%* Explain the manipulation

\subsection{Additional findings}
\Aviad{[ABE COMMENT] This whole (sub)section could be removed - the three-step description is redundant to what is above, and it looks like the efficiency section isn't really present }
\subsubsection{Zero clearing error}

We highlight that our algorithm described in Contribution I is not only fast - it also finds allocations with {\em zero} clearing error. Even the non-algorithmic existence proof of~\cite{Budish2011} only guarantees a {\em small} clearing error. Although this is the same algorithm as described above, we highlight it as a separate contribution because it is very important in practice. In real instances of allocating seats to students, undersubscribed courses are undesirable (economic inefficiency), but oversubscribed courses are often strictly forbidden (e.g.~due to classroom safety concerns). 

Previously, \cite{BudishCKO17} proposes  a practical but cumbersome workaround to the issue of oversubscribed courses; their procedure consists of three stages: (i) The first stage  simply runs the benchmark described above; by the time it terminates (\cite{BudishCKO17} use a 48 hours cutoff), it finds an approximate equilibrium, with small but nonzero clearing error. (ii) The second stage iteratively increases the prices of oversubscribed courses; while it eliminates oversubscription, higher prices causer more undersubscription, increasing the total clearing error increases in this stage. (iii) Finally in the third stage to compensate for undersubscription, the budgets of a subset of students is increased by 10\% so they can be more of the undersubscribed courses (but they're not allowed to add full courses to their schedules. The addition of second and third stage both complicates the mechanism and introduces inefficiencies and potential for strategic manipulation. Our approach completely avoids those stages because we obtain zero clearing error in the first place.   

\subsubsection{improved welfare}
Although our main focus is on improving the algorithmic efficiency and incentives guarantees of the A-CEEI mechanisms, in Section~\ref{sec:econeff} we compare the social welfare of our algorithm and the previous approach. Although the results aren't as decisive as on other metrics, we observe that our algorithm tends to give better allocations in terms of (utilitarian and Nash) social welfare.

\subsection{Limitations of our approach}
\paragraph{Modeling students' valuations} Throughout the paper we take students' reported preferences as their true valuations. In practice, students do not perfectly report their full preferences~\cite{Budish-Kessler-TBD}. In fact, students usually have a limited interface, e.g. they may rate courses as ``favourite, great, good, fair'', and there is algorithm hand-crafted conversion from those ratings to utilities. Concurrent work by~\cite{SZWS23} focuses on the  orthogonal direction of better modeling of students preferences using neural networks. Equilibrium computation is a major bottleneck of their approach, and we leave it to future work to see if our respective algorithms can be combined effectively.

\paragraph{Variance across markets} We are very fortunate to be able to test our algorithms on real data from a few different programs shared with us by Cognomos. There seem to be large variance between instances from different programs. In particular, in one school we find significant manipulations for the no-EF-TB and classic-EF-TB constraints, whereas in others those variants were also hard to manipulate. Running times also vary greatly between instances. However, two trends are consistent between all the instances we tested: (i) our algorithm is much faster than the previous state of the art, and (ii) robust EF-TB seems to have desirable incentive properties. We plan to test on more datasets as they become available. 

\paragraph{Limitations of the manipulation finding algorithm}
Our algorithm for discovering profitable manipulations is a highly imperfect surrogate to the real question of {\em can real students find robust manipulations?} On one hand, students can come up with more complicated manipulations than the ones considered by our algorithm; on the other hand, the algorithm has more information than any single student would normally have.  A particular issue is that we run our experiment for exploring profitable deviations with very small sample sizes: even with a very fast algorithm and restriction to very simple manipulations, we have to restrict our experiment to a as few as five samples, which is quite noisy. (We later validate every candidate manipulation with at least 100 iterations.) To make sure that our manipulation-finding algorithm still makes sense, we benchmark it on the HBS mechanism which is known to be manipulable~\cite{TBD}; indeed we find significant manipulations are possible with HBS on all instances. 


\subsection{Related work}

Equity stuff

Lots of recent work on fair division
